Neural Priming for Sample-Efficient Adaptation

We propose Neural Priming, a technique for adapting large pretrained models to distribution shifts and downstream tasks given few or no labeled examples. Presented with class names or unlabeled test samples, Neural Priming enables the model to recall and conditions its parameters on relevant data seen throughout pretraining, thereby priming it for the test distribution. Neural Priming can be performed at test time, even for pretraining datasets as large as LAION-2B. Performing lightweight updates on the recalled data significantly improves accuracy across a variety of distribution shift and transfer learning benchmarks. Concretely, in the zero-shot setting, we see a 2.45% improvement in accuracy on ImageNet and 3.81% accuracy improvement on average across standard transfer learning benchmarks. Further, using Neural Priming at inference to adapt to distribution shift, we see a 1.41% accuracy improvement on ImageNetV2. These results demonstrate the effectiveness of Neural Priming in addressing the challenge of limited labeled data and changing distributions. Code is available at github.com/RAIVNLab/neural-priming.

==> 2_Introduction.tex <==

\section{Introduction}
\label{sec:Introduction}

Training general-purpose models such as CLIP and ALIGN have emerged as the prevailing paradigm for reducing the reliance on task-specific data and improving performance. Though these large-scale models are trained on massive, diverse datasets, their performance often substantially improves when fine-tuned on task-specific data. This raises the question: Why does the model gain significant knowledge from fine-tuning on the target dataset, despite training on thousands of similar images throughout pretraining? 

One likely explanation for the observed improvements in model performance when fine-tuning on downstream data is the alignment between the fine tuning set and the test set, as they share the same distribution of labels and pixels. This alignment potentially enables the model to optimize for specific features that are unique to the target distribution, greatly improving its performance on the downstream task. Another potential factor lies in the sheer size of the pre-training dataset. The vast amount of data makes it challenging for the model to find a consistent solution that is optimal for all subsets of the data. Particularly for open-vocabulary models like CLIP, where many natural language descriptions can map to a single image, the challenge of accommodating all interpretations becomes apparent.\vivek{make this the main point}
\ani{How about -- One likely explanation for the observed improvements in model performance when fine-tuning on downstream data is the alignment between the fine tuning set and the test set, as both have the same distribution of labels and pixels.}\matt{That's great, I'll swap it in.}


To address the limitation of large-scale models to optimally model all subsets of the pre-training data, we turn to the concept of priming \cite{meyer1971facilitation} for inspiration. Priming refers to the activation of related information or schemas in human brains, leading to faster and more accurate processing and inference \cite{roediger}. When primed, our cognitive systems become attuned to specific concepts or stimuli, allowing us to retrieve and process relevant information more efficiently. For example, when presented with the word "dog," our semantic networks activate associated concepts such as "paws," or "barking," facilitating the recognition and comprehension of dog-related information. This priming effect occurs due to the activation and strengthening of neural connections between related concepts in our brains.

Drawing parallels to large-scale pretrained models, the concept of priming in humans offers insights into how such models can leverage prior knowledge and related information to improve their performance. Large models, which are trained on massive datasets, can be seen as analogous to the knowledge and associations encoded in human cognition. Similarly, conditioning models on recalled data from the pretrain set can be considered as a form of priming, aligning the model's knowledge with domain specific requirements.


With this in consideration, we propose a novel method, Neural Priming for sample-efficient transfer learning. Specifically Neural Priming recalls a subset of the pre-training data similar to the target distribution, re-aligns the natural language descriptions to the downstream task, and quickly adapts the model to the subset. Even for pre-training datasets containing 2 billion images, we can prime our model using previously seen data to a downstream task in seconds. We perform extensive experiments with CLIP models pre-trained on the LAION-2B datasets. We find Neural Priming leads to significant accuracy improvements, particularly in specialized domains. We demonstrate this approach on various transfer learning benchmarks, and observe an average improvement of 4.55\% zero-shot accuracy across standard benchmarks and notably a 9.60\% improvement on the fine-grained data set Oxford Flowers. These findings suggest that the large-scale models possess latent understanding of previously learned classes, and by recalling relevant data, the model can be primed for a specific task.

Moreover, our results highlight the effectiveness of Neural Priming when dealing with limited in-distribution training examples. By leveraging this approach, the model achieves comparable performance with far fewer samples. For instance, on the StanfordCars dataset, Neural Priming matches 10-shot accuracy without using any target training data. This demonstrates the potential of Neural Priming to improve sample-efficiency for general purpose models in transfer learning settings.


We make the following contributions:
\begin{itemize}
    \item 
        We propose a novel method, Neural Priming, which improves zero-shot and few-shot accuracy of CLIP models. Concretely we show a 3.81\% improvement in zero-shot accuracy on ImageNet, and as much as 9.27\% zero-shot accuracy improvement on Flowers102.
    
    
\end{itemize}

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{Figures/reservoir_figs.pdf}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}

% Given information about a new task either through natural language description or sample images, the model can introspect on previously seen data and prime its parameters for the task. 

% Priming theory suggests that related schema, or units of information stored in long-term memory, tend to activate simultaneously. This act of priming, or drawing related information into short-term memory, enables more accurate inference and recall. For example, the schema of rainstorms and slick roads may be linked closely in memory. Therefore, when someone perceives rain while driving, information relevant to slick roads is easily recalled and the driver knows to drive cautiously. 


% leads to schemas being activated in unison. Chains of related or connected information are activated and thus faster to recall into memory.  



% At inference the model receives a test image. The model recalls similar images from its pretrain set which are similar to the test data. Optimizing the model parameters on this relevant subset of the pretrain data significantly improves performance on a broad set of transfer learning and distribution shift datasets.    

%Introspective inference

==> neurips2023.tex <==
\begin{document}


\end{document}
